Bounding normalization time through intersection types

Non-idempotent intersection types are used in order to give a bound of the length of the normalization beta-reduction sequence of a lambda term: namely, the bound is expressed as a function of the size of the term.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{S. Graham-Lengrand and L. Paolini (Eds.): Sixth Workshop on\\ Intersection Types and Related Systems (ITRS 2012).\\
EPTCS 121, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.121.4}{10.4204/EPTCS.121.4}}

